Generalization Performance of Transfer Learning: Overparameterized and Underparameterized Regimes

Transfer learning is a useful technique for achieving improved performance and reducing training costs by leveraging the knowledge gained from source tasks and applying it to target tasks. Assessing the effectiveness of transfer learning relies on understanding the similarity between the ground truth of the source and target tasks. In real-world applications, tasks often exhibit partial similarity, where certain aspects are similar while others are different or irrelevant. To investigate the impact of partial similarity on transfer learning performance, we focus on a linear regression model with two distinct sets of features: a common part shared across tasks and a task-specific part. Our study explores various types of transfer learning, encompassing two options for parameter transfer. By establishing a theoretical characterization on the error of the learned model, we compare these transfer learning options, particularly examining how generalization performance changes with the number of features/parameters in both underparameterized and overparameterized regimes. Furthermore, we provide practical guidelines for determining the number of features in the common and task-specific parts for improved generalization performance. For example, when the total number of features in the source task's learning model is fixed, we show that it is more advantageous to allocate a greater number of redundant features to the task-specific part rather than the common part. Moreover, in specific scenarios, particularly those characterized by high noise levels and small true parameters, sacrificing certain true features in the common part in favor of employing more redundant features in the task-specific part can yield notable benefits.

==> proof_transfer_samples.tex <==
\section{Proof of Theorem~\ref{th.transfer_samples}}\label{app.proof_transfer_samples}

The formal statement of \cref{th.transfer_informal} is given by the following \cref{th.transfer_samples_similar}.
\begin{theorem}\label{th.transfer_samples_similar}
We have
\begin{align*}
    \E_{\ZZ,\ZZZ,\eOne,\eTwo}[\modelErr]=\KBias+\KNoise+\KSimilar,
\end{align*}
where in the overparameterized regime ($\pCommon > \nSum + 1$)
\begin{align*}
    &\E_{\XX,\XXX} \KBias =\left(1-\frac{\nSum}{\pCommon}\right)\normTwo{\wTwo}^2+\normTwo{\qTwo}^2,\\
    &\E_{\XX,\XXX} \KNoise=\frac{\nOne\left(\sigmaOne^2+\normTwo{\qOne}^2\right)+\nTwo\left(\sigmaTwo^2+\normTwo{\qTwo}^2\right)}{\pCommon-\nSum-1},\\
    &\Pr_{\XX,\XXX}\left\{\KSimilar\in\RangeKSimilar \right\}\\
    &\qquad \geq 1-\frac{4}{\nOne},
\end{align*}
and in the underparameterized regime ($\nSum > \pCommon + 1$),
\begin{align*}
    &\KBias = \normTwo{\qTwo}^2,\\
    &\E_{\XX,\XXX} \KNoise= \frac{\pCommon\left(\nOne\left(\sigmaOne^2+\normTwo{\qOne}^2\right)+\nTwo\left(\sigmaTwo^2+\normTwo{\qTwo}^2\right)\right)}{\nSum\left(\nSum-\pCommon-1\right)},\\
    &\Pr\left\{\KSimilar \leq \frac{\left(\nOne+2\sqrt{\nOne\ln \nOne}+2\ln \nOne\right)\similarity^2}{\left(\sqrt{\nSum}-\sqrt{\pCommon}-\sqrt{2\ln \nSum}\right)^2}\right\}\geq 1 - \frac{4}{\nOne}.
\end{align*}
\end{theorem}
Ignoring the logarithm terms and keeping the dominating terms in \cref{th.transfer_samples_similar}, we can get \cref{th.transfer_informal}. The proof of \cref{th.transfer_samples_similar} is in \cref{app.proof_transfer_samples_similar}.
% For the $\nOne$ samples for the source task, we define the corresponding input on $\featureSpaceSelected{2}$ as $\ZFake\in \mathds{R}^{\pSpecial{2}\times \nOne}$ and the corresponding input on $\featureSpace{1}$ as $\ZTrue\in \mathds{R}^{s_1\times \nOne}$. By \cref{as.orthogonal}, we know that $\ZFake$ is independent of $\ZTrue$. By \cref{eq.ground_truth_original}, we have
% \begin{align}
    % \yOne= \XX^T\wOne + \ZTrue^T\sq{1} + \eOne.\label{eq.temp_012505}
% \end{align}


\section{Proof of Theorem~\ref{th.transfer_samples_similar}}\label{app.proof_transfer_samples_similar}

We define
\begin{align}
    &\VV\defeq \myMa{\XX &\XXX}\in \mathds{R}^{\pCommon\times \nSum},\label{eq.def_V}\\
    &\eTilde\defeq \myMa{\ZZ^T\qOne+\eOne\\\ZZZ^T\qTwo+\eTwo}\in \mathds{R}^{\nSum},\label{eq.def_eTilde}\\
    &\xiTerm \defeq \myMa{\XX^T(\wOne-\wTwo)\\\bm{0}}\in \mathds{R}^{\nSum}\label{eq.def_xi}.
\end{align}
By \cref{as.Gaussian}, we have
\begin{align}
    \eTilde\sim \mathcal{N}\left(\bm{0},\ \diag\left(\underbrace{\sigmaOne^2+\normTwo{\qOne}^2,\cdots}_{ \nOne \text{ terms}},\underbrace{\sigmaTwo^2+\normTwo{\qTwo}^2,\cdots}_{\nTwo\text{ terms}}\right)\right).\label{eq.temp_012510}
\end{align}
By \cref{eq.def_xi} and \cref{as.Gaussian}, we have
\begin{align*}
    \xiTerm_{1:\nOne} \sim \mathcal{N}(\bm{0},\similarity^2\iMatrix{\nOne}) \text{ (recall the definition of $\similarity$ in \cref{eq.def_similarity})},
\end{align*}
where $\xiTerm_{1:\nOne}$ denotes the vector that consists of the first $\nOne$ elements of $\xiTerm$.
Thus, we know that $\normTwo{\xiTerm_{1:\nOne}}^2/\similarity^2$ follows $\chi^2$ distribution with $\nOne$ degrees of freedom. Also notice that $\normTwo{\xiTerm}=\normTwo{\xiTerm_{1:\nOne}}$ (recalling the definition of $\xiTerm$ in \cref{eq.def_xi}). Thus, by \cref{le.chi_bound}, we have
\begin{align}
    \Pr\left\{\frac{\normTwo{\xiTerm}^2}{\similarity^2}\in \left[\nOne-2\sqrt{\nOne\ln \nOne},\ \nOne+2\sqrt{\nOne\ln \nOne}+2\ln \nOne\right]\right\}\geq 1- \frac{2}{\nOne}.\label{eq.temp_022101}
\end{align}
By \cref{eq.ground_truth_matrix},  we have
\begin{align*}
    \myMa{\yOne\\\yTwo}=&\myMa{\XX^T\wOne+\ZZ^T\qOne+\eOne\\\XXX^T\wTwo+\ZZZ^T\qTwo+\eTwo}\\
    % =&\myMa{\XX^T\wTwo+\ZFake^T\qTwo\\\XXX^T\wTwo+\ZZZ^T\qTwo}+\eTilde\text{ (since $\wOne=\wTwo$ by \cref{as.orthogonal})}\\
    =&\VV^T \wTwo+\xiTerm+\eTilde\ \text{ (by \cref{eq.def_V,eq.def_eTilde,eq.def_xi})}.\numberthis \label{eq.temp_012506}
\end{align*}


\subsection*{The overparameterized situation}
The min $\ell_2$-norm overfitted solution is
\begin{align*}
    \wTildeTwo
    =&\VV(\VV^T\VV)^{-1}\myMa{\yOne\\\yTwo}\\
    =&\VV(\VV^T\VV)^{-1}\VV^T\wTwo+ \VV(\VV^T\VV)^{-1}\xiTerm + \VV(\VV^T\VV)^{-1} \eTilde\ \text{ (by \cref{eq.temp_012506})}.\numberthis \label{eq.temp_040501}
\end{align*}
Thus, we have
\begin{align*}
    \modelErr=&\normTwo{\myMa{\wTildeTwo\\\qTilde}-\myMa{\wTwo\\\qTwo}}^2\text{ (by \cref{eq.def_model_err})}\\
    =&\normTwo{\wTildeTwo-\wTwo}^2 + \normTwo{\qTwo}^2\text{ (since $\qTilde=\bm{0}$)}\\
    =&\normTwo{\left(\iMatrix{\pCommon}-\VV(\VV^T\VV)^{-1}\VV^T\right)\wTwo+\VV(\VV^T\VV)^{-1}\xiTerm + \VV(\VV^T\VV)^{-1} \eTilde}^2 + \normTwo{\qTwo}^2\ \text{ (by \cref{eq.temp_040501})}.\numberthis \label{eq.temp_012507}
\end{align*}
Notice that
\begin{align*}
    \left(\iMatrix{\pCommon}-\VV(\VV^T\VV)^{-1}\VV^T\right)^T \VV(\VV^T\VV)^{-1}=\VV(\VV^T\VV)^{-1}-\VV(\VV^T\VV)^{-1}=0.
\end{align*}
Thus, by expanding \cref{eq.temp_012507}, the term of the inner product between $\left(\iMatrix{\pCommon}-\VV(\VV^T\VV)^{-1}\VV^T\right)\wTwo$ and $\VV(\VV^T\VV)^{-1}\xiTerm + \VV(\VV^T\VV)^{-1} \eTilde$ equals to zero. Thus, we have
\begin{align}
    \modelErr =& \normTwo{\left(\iMatrix{\pCommon}-\VV(\VV^T\VV)^{-1}\VV^T\right)\wTwo}^2+\normTwo{\VV(\VV^T\VV)^{-1}\xiTerm + \VV(\VV^T\VV)^{-1} \eTilde}^2+\normTwo{\qTwo}^2.\label{eq.temp_012508}
\end{align}
We have
\begin{align*}
    &\E_{\substack{\XX,\XXX, \\ \ZZ,\ZZZ,\\ \eOne,\eTwo}}\normTwo{\VV(\VV^T\VV)^{-1}\eTilde}^2\\
    =&\E_{\VV,\eTilde} [\eTilde^T(\VV^T\VV)^{-1} \eTilde]\\
    =&\E_{\eTilde}[\eTilde^T\E_{\VV}[(\VV^T\VV)^{-1}] \eTilde]\text{ (since $\VV$ and $\eTilde$ are independent)}\\
    =&\frac{\E\limits_{\eTilde}[\eTilde^T\eTilde]}{\pCommon-\nSum-1}\text{ (by \cref{le.IW})}\\
    =&\frac{\nOne\left(\sigmaOne^2+\normTwo{\qOne}^2\right)+\nTwo\left(\sigmaTwo^2+\normTwo{\qTwo}^2\right)}{\pCommon-\nSum-1}\text{ (by \cref{eq.temp_012510})}.\numberthis \label{eq.temp_012511}
\end{align*}
When $\wOne=\wTwo$, by \cref{eq.temp_012508}, we have
\begin{align*}
    &\E[\modelErr]\\
    =&\E\normTwo{\left(\iMatrix{\pCommon}-\VV(\VV^T\VV)^{-1}\VV^T\right)\wTwo}^2+\E\normTwo{\VV(\VV^T\VV)^{-1} \eTilde}^2+\normTwo{\qTwo}^2\\
    &\text{ (by \cref{eq.def_xi}, we have $\xiTerm=\bm{0}$ when $\wOne=\wTwo$)}\\
    =& \left(1-\frac{\nSum}{\pCommon}\right)\normTwo{\wTwo}^2+\frac{\nOne\left(\sigmaOne^2+\normTwo{\qOne}^2\right)+\nTwo\left(\sigmaTwo^2+\normTwo{\qTwo}^2\right)}{\pCommon-\nSum-1}+\normTwo{\qTwo}^2\\
    &\text{ (by \cref{le.bias} and \cref{eq.temp_012511})}. \numberthis \label{eq.temp_041003}
\end{align*}
(The expectation in \cref{eq.temp_041003} is on all random variables $\XX,\XXX,\ZZ,\ZZZ,\eOne,\eTwo$.)

When $\wOne\neq \wTwo$, since $\E[\eTilde]=\bm{0}$ and is independent of $\VV$ and $\xiTerm$ by \cref{as.Gaussian}, we have
\begin{align}
    \E_{\eTilde}\normTwo{\VV(\VV^T\VV)^{-1}\xiTerm + \VV(\VV^T\VV)^{-1} \eTilde}^2=\normTwo{\VV(\VV^T\VV)^{-1}\xiTerm}^2+\E_{\eTilde}\normTwo{\VV(\VV^T\VV)^{-1} \eTilde}^2.\label{eq.temp_040601}
\end{align}
It remains to estimate $\normTwo{\VV(\VV^T\VV)^{-1}\xiTerm}^2$. To that end, we have
\begin{align*}
    \normTwo{\VV(\VV^T\VV)^{-1}\xiTerm}^2=&\xiTerm^T(\VV^T\VV)^{-1}\xiTerm\\
    \in & \left[\frac{\normTwo{\xiTerm}^2}{\max\eig(\VV^T\VV)},\ \frac{\normTwo{\xiTerm}^2}{\min\eig(\VV^T\VV)}\right]\\
    =&\left[\frac{\normTwo{\xiTerm}^2}{\lambda_{\max}^2(\VV)}, \frac{\normTwo{\xiTerm}^2}{\lambda_{\min}^2(\VV)}\right].\numberthis \label{eq.temp_022103}
\end{align*}
By \cref{le.singular_Gaussian} (by letting $t=\sqrt{2\ln \nOne}$), we have
\begin{align}
    \Pr\left\{\sqrt{\pCommon}-\sqrt{\nSum}-\sqrt{2\ln \nOne}\leq \lambda_{\min}(\VV)\leq \lambda_{\max}(\VV)\leq \sqrt{\pCommon}+\sqrt{\nSum}+\sqrt{2\ln \nOne}\right\}\geq 1 - \frac{2}{\nOne}.\label{eq.temp_022102}
\end{align}
Plugging \cref{eq.temp_022102,eq.temp_022101} into \cref{eq.temp_022103} by the union bound, we thus have
\begin{align*}
    &\Pr\left\{\normTwo{\VV(\VV^T\VV)^{-1}\xiTerm}^2\in \RangeKSimilar\right\}\\
    &\geq 1- \frac{4}{\nOne}.
\end{align*}



\subsection*{The underparameterized situation}
The solution that minimizes the training loss is
\begin{align*}
    \wTildeTwo=&(\VV\VV^T)^{-1}\VV\myMa{\yOne\\\yTwo}\\
    =&(\VV\VV^T)^{-1}\VV\left(\VV^T \wTwo+\xiTerm+\eTilde\right)\text{ (by \cref{eq.temp_012506})}\\
    =&\wTwo+(\VV\VV^T)^{-1}\VV\xiTerm + (\VV\VV^T)^{-1}\VV\eTilde.\numberthis \label{eq.temp_041004}
\end{align*}
Thus, we have
\begin{align*}
    \modelErr =& \normTwo{\wTildeTwo-\wTwo}^2+\normTwo{\qTilde-\qTwo}^2\ \text{ (by \cref{eq.def_model_err})}\\
    =&\normTwo{\wTildeTwo-\wTwo}^2 + \normTwo{\qTwo}^2\ \text{ (since $\qTilde=\bm{0}$)}\\
    =&\normTwo{\qTwo}^2 + \normTwo{(\VV\VV^T)^{-1}\VV\xiTerm + (\VV\VV^T)^{-1}\VV\eTilde}^2\ \text{ (by \cref{eq.temp_041004})}
\end{align*}
When $\similarity=0$, we have
\begin{align*}
    \E_{\substack{\XX,\XXX, \\ \ZZ,\ZZZ,\\ \eOne,\eTwo}}[\modelErr] = &\normTwo{\qTwo}^2+\E_{\substack{\XX,\XXX, \\ \ZZ,\ZZZ,\\ \eOne,\eTwo}}\normTwo{(\VV\VV^T)^{-1}\VV\eTilde}^2\\
    =& \normTwo{\qTwo}^2+ \frac{\pCommon\left(\nOne\left(\sigmaOne^2+\normTwo{\qOne}^2\right)+\nTwo\left(\sigmaTwo^2+\normTwo{\qTwo}^2\right)\right)}{\nSum\left(\nSum-\pCommon-1\right)}\\
    &\text{ (by \cref{le.IW} and \cref{eq.temp_012510})}.
\end{align*}
When $\similarity\neq 0$, similar to \cref{eq.temp_040601}, we have
\begin{align*}
    \E_{\eTilde}\normTwo{(\VV^T\VV)^{-1}\VV\xiTerm + (\VV^T\VV)^{-1} \VV\eTilde}^2=\normTwo{(\VV^T\VV)^{-1}\VV\xiTerm}^2+\E_{\eTilde}\normTwo{(\VV^T\VV)^{-1} \VV\eTilde}^2.
\end{align*}

We have
\begin{align}
    \normTwo{(\VV^T\VV)^{-1}\VV\xiTerm}^2 \leq \frac{\normTwo{\xiTerm}^2}{\lambda_{\min}^2(\VV)}\ \text{ (by \cref{le.norm_min_eig})}.\label{eq.temp_041001}
\end{align}
By \cref{le.singular_Gaussian} and \cref{as.Gaussian}, we have
\begin{align}
    \Pr\left\{\lambda_{\min}(\VV)\geq \sqrt{\nSum}-\sqrt{\pCommon}-\sqrt{2\log \nSum}\right\}\geq 1-\frac{2}{\nSum}.\label{eq.temp_041002}
\end{align}
By \cref{eq.temp_022101,eq.temp_041001,eq.temp_041002} and the union bound, we have
\begin{align*}
    &\Pr\left\{\normTwo{(\VV^T\VV)^{-1}\VV\xiTerm}^2 \leq \frac{\left(\nOne+2\sqrt{\nOne\ln \nOne}+2\ln \nOne\right)\similarity^2}{\left(\sqrt{\nSum}-\sqrt{\pCommon}-\sqrt{2\log \nSum}\right)^2}\right\}\\
    \geq &1 - \frac{2}{\nOne}-\frac{2}{\nSum}\\
    \geq & 1 - \frac{4}{\nOne}.
\end{align*}

\section{With fine-tuning}
In this situation, we are using $\pSpecial{2}$ features to fit $\nTwo$ samples. Depending on whether $\pSpecial{2}$ or $\nTwo$ is larger, we also have overparameterized and underparameterized fine-tuning situations.

\newcommand{\CC}{C_{\sigmaOne,\sigmaTwo,\qOne,\qTwo,\similarity}}
Define
\begin{align*}
    &\kTilde\defeq  \frac{ \pCommon + 2\sqrt{ \pCommon\ln \pCommon} + 2\ln \pCommon}{\nSum - 2\sqrt{\nSum \ln \nSum}},\numberthis \label{eq.def_kTilde}\\
    &\CC\defeq 3\left(\tilde{k}\sigmaOne^2 + \tilde{k}\normTwo{\qOne}^2+\similarity^2\right) \left(\nOne+2\sqrt{\nOne\ln \nOne}+2\ln \nOne\right)\\
    &\qquad + 3\left(\sigmaTwo^2 +\tilde{k}\sigmaTwo^2+\tilde{k} \normTwo{\qTwo}^2\right)\left(\nTwo+2\sqrt{\nTwo\ln \nTwo}+2\ln \nTwo\right)\numberthis \label{eq.def_CC}.
\end{align*}

\section{Proof of Corollary~\ref{coro.fine_tune}}\label{proof.coro_fine_tune}

If we ignore those logarithm terms in \cref{eq.def_kTilde,eq.def_CC}, we can approximate $\CC$ by $A$ defined in \cref{eq.def_Q}.


\begin{lemma}
If $\nTwo\geq 5000$, and $\nTwo \in \left[60 \sqrt{\pSpecial{2}\ln \pSpecial{2}},\ \frac{\pSpecial{2}}{500}\right]$, then
\begin{align*}
    & \left(\sqrt{\pSpecial{2}}-\sqrt{\nTwo}-\sqrt{2\ln \nTwo}\right)^2 \geq 0.9 \pSpecial{2},\numberthis \label{eq.temp_050101}\\
    & \frac{\pSpecial{2}-\nTwo + 2\sqrt{(\pSpecial{2}-\nTwo)\ln \pSpecial{2}}+2\ln \pSpecial{2}}{\pSpecial{2}-2\sqrt{\pSpecial{2}\ln \pSpecial{2}}} \leq 1 - 0.9\frac{\nTwo}{\pSpecial{2}}.\numberthis \label{eq.temp_050102}
\end{align*}
If $\nTwo \geq 500\pSpecial{2}$ and $\pSpecial{2}\geq 5000$, then
\begin{align}
    \left(\sqrt{\nTwo}-\sqrt{\pSpecial{2}}-\sqrt{2\ln \pSpecial{2}}\right)^2 \geq 0.9 \nTwo.\label{eq.temp_050103}
\end{align}
\end{lemma}
\begin{proof}
We have
\begin{align*}
    &\pSpecial{2}\geq 500 \nTwo\\
    \implies & \frac{\nTwo}{\pSpecial{2}}\leq \left(\frac{1-\sqrt{0.9}}{1.1}\right)^2\ \text{ (since $\left(\frac{1-\sqrt{0.9}}{1.1}\right)^2\approx 0.00218\leq \frac{1}{500}$)}\\
    \implies & 1.1\sqrt{\nTwo}\leq\left( 1-\sqrt{0.9}\right)\sqrt{\pSpecial{2}}\\
    \implies & \sqrt{\nTwo}+0.1\sqrt{2\ln \nTwo} \leq \left( 1-\sqrt{0.9}\right)\sqrt{\pSpecial{2}}\\
    &\text{ (since $\frac{\nTwo}{\ln \nTwo}\geq 200=\frac{2}{0.1^2}$ when $\nTwo\geq 5000$, by noticing that $\frac{5000}{\ln 5000}\approx 587$)}\\
    \implies & \text{\cref{eq.temp_050101}}.
\end{align*}
We also have
\begin{align*}
    &\nTwo \geq 60 \sqrt{\pSpecial{2}\ln \pSpecial{2}}\\
    \implies & 0.1\nTwo \geq 6 \sqrt{\pSpecial{2}\ln \pSpecial{2}}\\
    \implies & \nTwo - 6\sqrt{\pSpecial{2}\ln \pSpecial{2}}\geq 0.9 \nTwo\\
    \implies & \frac{\nTwo - 6\sqrt{\pSpecial{2}\ln \pSpecial{2}}}{\pSpecial{2}}\geq 0.9\frac{\nTwo}{\pSpecial{2}}\\
    \implies & \frac{\nTwo - 6\sqrt{\pSpecial{2}\ln \pSpecial{2}}}{\pSpecial{2}-2\sqrt{\pSpecial{2}\ln \pSpecial{2}}}\geq 0.9 \frac{\nTwo}{\pSpecial{2}}\\
    &\text{ (the denominator is positive when $\pSpecial{2} > 16$)}\\
    \implies & \frac{\nTwo-2\sqrt{(\pSpecial{2}-\nTwo)\ln \pSpecial{2}} - 2\ln \pSpecial{2} - 2\sqrt{\pSpecial{2}\ln \pSpecial{2}}}{\pSpecial{2}-2\sqrt{\pSpecial{2}\ln \pSpecial{2}}}\geq 0.9 \frac{\nTwo}{\pSpecial{2}}\\
    & \text{ (since $\pSpecial{2}-\nTwo\leq \pSpecial{2}$ and $\ln \pSpecial{2}< \pSpecial{2}$ when $\pSpecial{2}>16$)}\\
    \implies & \text{\cref{eq.temp_050102}}.
\end{align*}
Similar to \cref{eq.temp_050101}, we have \cref{eq.temp_050103}. The result of this lemma thus follows.
\end{proof}


\begin{lemma}\label[lemma]{le.fine_CC}
If $\nOne,\nTwo\geq 5000$, $\pCommon>4286$, $\frac{\pCommon}{\nSum}\leq \frac{1}{7}$, and \cref{eq.requirement}, then
\begin{align*}
    \CC \leq \frac{7}{12}\nTwo\normTwo{\qTwo}^2.
\end{align*}
\end{lemma}
Proof of \cref{le.fine_CC} is in \cref{subsec.proof_fine_CC}.


\begin{proof}
\begin{align*}
    1-\frac{0.9 \nTwo}{\pSpecial{2}} + \frac{7}{12}\cdot \frac{\nTwo}{0.9\pSpecial{2}}\approx 1- 0.2519 \frac{\nTwo}{\pSpecial{2}}\leq 1 -\frac{\nTwo}{4\pSpecial{2}}.
\end{align*}

\begin{align*}
    \frac{7}{12}\cdot \frac{1}{0.9}\approx 0.648\leq 0.65
\end{align*}
\TODO
\end{proof}

\begin{theorem}\label{th.fine_tune}
After fine-tuning in the underparameterized regime ($\pCommon< \nSum + 1$), $\KNoise$ and $\KSimilar$ in \cref{th.transfer_samples_similar} do not change, while the term $\KBias$ becomes
\begin{align*}
    \KBias^{\text{fine-tuning}}=\TBias + \TVar,
\end{align*}
where in the overparameterized fine-tuning regime ($\pSpecial{2}> \nTwo+1$)
\begin{align*}
    &\E[\TBias] = \left(1 - \frac{\nTwo}{\pSpecial{2}}\right)\normTwo{\qTwo}^2,\numberthis \label{eq.temp_042701}\\
    &\Pr\left\{\TBias\leq \frac{\pSpecial{2}-\nTwo + 2\sqrt{(\pSpecial{2}-\nTwo)\ln \pSpecial{2}}+2\ln \pSpecial{2}}{\pSpecial{2}-2\sqrt{\pSpecial{2}\ln \pSpecial{2}}}\normTwo{\qTwo}^2\right\}\geq 1 - \frac{2}{\pSpecial{2}},\numberthis \label{eq.temp_042702}\\
    &\Pr\left\{\TVar\leq \frac{\CC}{\left(\sqrt{\pSpecial{2}}-\sqrt{\nTwo}-\sqrt{2\ln \nTwo}\right)^2}\right\}\geq 1 - \frac{10}{\min \{\nOne,\nTwo,\pCommon\}},\numberthis \label{eq.temp_042703}
\end{align*}
and in the underparameterized fine-tuning regime ($\nTwo > \pSpecial{2} + 1$)
\begin{align*}
    &\TBias = 0,\\
    &\Pr\left\{\TVar\leq \frac{\CC}{\left(\sqrt{\nTwo}-\sqrt{\pSpecial{2}}-\sqrt{2\log \nTwo}\right)^2}\right\}\geq 1 - \frac{10}{\min \{\nOne,\nTwo,\pCommon,\pSpecial{2}\}}.
\end{align*}
\end{theorem}
The proof of \cref{th.fine_tune} is in the following two subsections.







\subsection{Overparameterized fine-tuning}
By \cref{le.min_l2_solution}, given $\wTildeTwo$, the learned result $\qTilde$ by GD/SGD from a zero initial point is the solution of the following optimization problem:
\begin{align*}
    \min_{\qHat}\quad  &\normTwo{\qHat}\\
    \text{subject to }\quad  & \yTwo=\XXX^T \wTildeTwo + \ZZZ^T \qHat.
\end{align*}
Thus, we have
\begin{align*}
    &\qTilde \\
    =& \ZZZ(\ZZZ^T\ZZZ)^{-1} \left(\yTwo - \XXX^T \wTildeTwo\right)\\
    = &\ZZZ(\ZZZ^T\ZZZ)^{-1}\left(\XXX^T\wTwo+\ZZZ^T\qTwo+\eTwo-\XXX^T\left(\wTwo+(\VV\VV^T)^{-1}\VV\xiTerm + (\VV\VV^T)^{-1}\VV\eTilde\right)\right)\\
    &\text{ (by \cref{eq.ground_truth_matrix,eq.temp_041004})}\\
    =& \ZZZ(\ZZZ^T\ZZZ)^{-1}\ZZZ^T \qTwo  + \ZZZ(\ZZZ^T\ZZZ)^{-1} \bm{\gamma},
\end{align*}
where
\begin{align}
    \bm{\gamma}\defeq \eTwo - \XXX^T(\VV\VV^T)^{-1}\VV\left(\xiTerm + \eTilde\right).\label{eq.def_gamma}
\end{align}
Thus, we have
\begin{align*}
    \qTilde-\qTwo=\left(\iMatrix{\pSpecial{2}}-\ZZZ(\ZZZ^T\ZZZ)^{-1}\ZZZ^T\right)\qTwo + \ZZZ(\ZZZ^T\ZZZ)^{-1} \bm{\gamma}
\end{align*}
Also because
\begin{align*}
    \left(\iMatrix{\pSpecial{2}}-\ZZZ(\ZZZ^T\ZZZ)^{-1}\ZZZ^T\right)^T \ZZZ(\ZZZ^T\ZZZ)^{-1}= 0.
\end{align*}
we thus have
\begin{align}
    \normTwo{\qTilde-\qTwo}^2 =& \normTwo{\left(\iMatrix{\pSpecial{2}}-\ZZZ(\ZZZ^T\ZZZ)^{-1}\ZZZ^T\right)\qTwo }^2 + \normTwo{\ZZZ(\ZZZ^T\ZZZ)^{-1} \bm{\gamma}}^2\nonumber\\
    =& \TBias + \TVar.\label{eq.temp_042401}
\end{align}
where we define
\begin{align*}
    &\TBias\defeq \normTwo{\left(\iMatrix{\pSpecial{2}}-\ZZZ(\ZZZ^T\ZZZ)^{-1}\ZZZ^T\right)\qTwo }^2,\\
    &\TVar\defeq \normTwo{\ZZZ(\ZZZ^T\ZZZ)^{-1} \bm{\gamma}}^2.
\end{align*}
By \cref{le.bias}, we have proven \cref{eq.temp_042701,eq.temp_042702}.
% \begin{align}
%     \E \normTwo{\left(\iMatrix{\pSpecial{2}}-\ZZZ(\ZZZ^T\ZZZ)^{-1}\ZZZ^T\right)\qTwo }^2 = \left(1 - \frac{\nTwo}{\pSpecial{2}}\right)\normTwo{\qTwo}^2.\label{eq.temp_042402}
% \end{align}
It remains to prove \cref{eq.temp_042703}, i.e., estimate the term $\normTwo{\ZZZ(\ZZZ^T\ZZZ)^{-1} \bm{\gamma}}^2$. To that end, we have
\begin{align*}
    \normTwo{\ZZZ(\ZZZ^T\ZZZ)^{-1} \bm{\gamma}}^2 \in &\left[\frac{\normTwo{\bm{\gamma}}^2}{\lambda_{\max}^2(\ZZZ)}, \frac{\normTwo{\bm{\gamma}}^2}{\lambda_{\min}^2(\ZZZ)}\right]\ \text{ (similar to \cref{eq.temp_022103})}.\numberthis \label{eq.temp_042307}
\end{align*}
By \cref{le.singular_Gaussian} (by letting $t=\sqrt{2\ln \nTwo}$), we have
\begin{align}
    &\Pr\left\{\sqrt{\pSpecial{2}}-\sqrt{\nTwo}-\sqrt{2\ln \nTwo}\leq \lambda_{\min}(\ZZZ)\leq \lambda_{\max}(\ZZZ)\leq \sqrt{\pSpecial{2}}+\sqrt{\nTwo}+\sqrt{2\ln \nTwo}\right\}\nonumber\\
    &\geq 1 - \frac{2}{\nTwo}.\label{eq.temp_042201}
\end{align}
It remains to estimate $\normTwo{\bm{\gamma}}^2$. To that end, we have
\begin{align*}
    \normTwo{\bm{\gamma}}=&\normTwo{\eTwo-\XXX^T(\VV\VV^T)^{-1}\VV\left(\xiTerm + \eTilde\right)}\\
    \leq &\normTwo{\eTwo} + \normTwo{\XXX^T(\VV\VV^T)^{-1}\VV\left(\xiTerm + \eTilde\right)} \ \text{ (by the triangle inequality)}\\
    \leq &  \normTwo{\eTwo} +\sqrt{\normTwo{\XXX^T(\VV\VV^T)^{-1}\VV\left(\xiTerm + \eTilde\right)}^2 + \normTwo{\XX^T(\VV\VV^T)^{-1}\VV\left(\xiTerm + \eTilde\right)}^2}\\
    =& \normTwo{\eTwo} +\sqrt{\normTwo{\myMa{\XX^T\\\XXX^T}(\VV\VV^T)^{-1}\VV\left(\xiTerm + \eTilde\right)}^2}\\
    = & \normTwo{\eTwo} +\normTwo{\VV^T(\VV\VV^T)^{-1}\VV\left(\xiTerm + \eTilde\right)}\ \text{ (by \cref{eq.def_V})}\\
    \leq & \normTwo{\eTwo} +\normTwo{\VV^T(\VV\VV^T)^{-1}\VV\xiTerm}+\normTwo{\VV^T(\VV\VV^T)^{-1}\VV\eTilde}\ \text{ (by the triangle inequality)}\\
    \leq & \normTwo{\eTwo} +\normTwo{\xiTerm} + \normTwo{\VV^T(\VV\VV^T)^{-1}\VV\eTilde}\ \text{ (since $\VV^T(\VV\VV^T)^{-1}\VV$ is a projection)}.
\end{align*}

Thus, we have
\begin{align*}
    &\normTwo{\bm{\gamma}}^2\\
    \leq & \left(\normTwo{\eTwo} +\normTwo{\xiTerm} + \normTwo{\VV^T(\VV\VV^T)^{-1}\VV\eTilde}\right)^2\\
    \leq & 3 \normTwo{\eTwo}^2 +3\normTwo{\xiTerm}^2 + 3\normTwo{\VV^T(\VV\VV^T)^{-1}\VV\eTilde}^2 \ \text{ (by the Cauchy–Schwarz inequality)}.\numberthis \label{eq.temp_042304}
\end{align*}


By \cref{eq.def_V,eq.def_eTilde} and \cref{as.Gaussian}, we know that $\VV$ and $\eTilde$ are independent of each other. Due to this independence, we can apply \cref{le.bias} and thus have
\begin{align}
    \Pr\left\{\normTwo{\VV^T(\VV\VV^T)^{-1}\VV\eTilde}^2 \leq \frac{ \pCommon + 2\sqrt{ \pCommon\ln \pCommon} + 2\ln \pCommon}{\nSum - 2\sqrt{\nSum \ln \nSum}}\normTwo{\eTilde}^2\right\}\geq 1 - \frac{1}{\nSum} - \frac{1}{\pCommon}.\label{eq.temp_042901}
\end{align}

Let $[\cdot]_{a_1:a_2}$ denote the sub-vector from $a_1$-th element to $a_2$-th element (inclusive endpoints).
By \cref{eq.def_eTilde,eq.temp_012510} and \cref{as.Gaussian}, we know that $\normTwo{[\eTilde]_{1:\nOne}}^2 / \left(\sigmaOne^2 + \normTwo{\qOne}^2\right)$ follows $\chi^2$ distribution with $\nOne$ degrees of freedom.
By \cref{le.chi_bound}, we have
\begin{align*}
    &\Pr\left\{\frac{\normTwo{[ \eTilde]_{1:\nOne}}^2}{\sigmaOne^2 + \normTwo{\qOne}^2}\in \left[\nOne-2\sqrt{\nOne\ln \nOne},\ \nOne+2\sqrt{\nOne\ln \nOne}+2\ln \nOne\right]\right\}\\
    &\geq 1- \frac{2}{\nOne}.\numberthis \label{eq.temp_042301}
\end{align*}
Similarly, we have
\begin{align*}
    &\Pr\left\{\frac{\normTwo{[\eTilde]_{\nOne+1:\nOne+\nTwo}}^2}{\sigmaTwo^2 + \normTwo{\qTwo}^2}\in \left[\nTwo-2\sqrt{\nTwo\ln \nTwo},\ \nTwo+2\sqrt{\nTwo\ln \nTwo}+2\ln \nTwo\right]\right\}\\
    &\geq 1- \frac{2}{\nTwo}.\numberthis \label{eq.temp_042302}
\end{align*}
By \cref{eq.temp_042901,eq.temp_042301,eq.temp_042302} and the union bound, we have
\begin{align}
    &\Pr\left\{\normTwo{\VV^T(\VV\VV^T)^{-1}\VV\eTilde}^2 \leq \tilde{k}\tilde{C}\right\}\nonumber\\
    \geq & 1- \frac{1}{\nSum}-\frac{1}{\pCommon}-\frac{2}{\nOne}-\frac{2}{\nTwo}\nonumber\\
    \geq & 1 - \frac{6}{\min \{\nOne,\nTwo,\pCommon\}},\label{eq.temp_042903}
\end{align}
where
\begin{align*}
    \tilde{C}\defeq & \left(\sigmaOne^2 + \normTwo{\qOne}^2\right)\left(\nOne + 2\sqrt{\nOne\ln \nOne}+2\ln \nOne\right)\\
    &+ \left(\sigmaTwo^2 + \normTwo{\qTwo}^2\right)\left(\nTwo+ 2\sqrt{\nTwo\ln \nTwo}+2\ln \nTwo\right).
\end{align*}

By \cref{as.Gaussian}, we know that $\normTwo{\eTwo}^2 / \sigmaTwo^2$ follows $\chi^2$ distribution with $\nTwo$ degrees of freedom. By \cref{le.chi_bound}, we have
\begin{align}
    \Pr\left\{\frac{\normTwo{\eTwo}^2}{\sigmaTwo^2}\in \left[\nTwo-2\sqrt{\nTwo\ln \nTwo},\ \nTwo+2\sqrt{\nTwo\ln \nTwo}+2\ln \nTwo\right]\right\}\geq 1 - \frac{2}{\nTwo}.\label{eq.temp_042303}
\end{align}


Plugging \cref{eq.temp_022101,eq.temp_042903,eq.temp_042303} into \cref{eq.temp_042304} by the union bound, we have
\begin{align*}
    &\Pr\bigg\{\normTwo{\bm{\gamma}}^2\leq\CC \bigg\}\geq 1 - \frac{8}{\min \{\nOne,\nTwo,\pCommon\}}.\numberthis \label{eq.temp_042305}
\end{align*}
By \cref{eq.temp_042305,eq.temp_042307,eq.temp_042201} and the union bound, we thus get \cref{eq.temp_042703}.
% \begin{align}
%     \Pr\left\{\normTwo{\ZZZ(\ZZZ^T\ZZZ)^{-1} \bm{\gamma}}^2\leq \frac{\CC}{\left(\sqrt{\pSpecial{2}}-\sqrt{\nTwo}-\sqrt{2\ln \nTwo}\right)^2}\right\}\geq 1 - \frac{4}{\nOne}- \frac{4}{\nTwo}.\label{eq.temp_042403}
% \end{align}
% The result in the overparameterized fine-tuning regime thus follows by \cref{eq.temp_042401,eq.temp_042402,eq.temp_042403}.

\subsection{Underparameterized situation}
Given $\wTildeTwo$, the fine-tuning result $\qTilde$ will minimize the training MSE (mean squared error), i.e.,
\begin{align*}
    \min_{\qHat} \normTwo{\yTwo - (\XXX\wTildeTwo + \ZZZ \qHat)}^2.
\end{align*}
Thus, we have
\begin{align*}
    &\qTilde\\
    =& (\ZZZ\ZZZ^T)^{-1}\ZZZ \left(\yTwo - \XXX\wTildeTwo\right)\\
    =& (\ZZZ\ZZZ^T)^{-1}\ZZZ\left(\XXX^T\wTwo+\ZZZ^T\qTwo+\eTwo-\XXX^T\left(\wTwo+(\VV\VV^T)^{-1}\VV\xiTerm + (\VV\VV^T)^{-1}\VV\eTilde\right)\right)\\
    &\text{ (by \cref{eq.ground_truth_matrix,eq.temp_041004})}\\
    =&\qTwo + (\ZZZ\ZZZ^T)^{-1}\ZZZ\left(\eTwo -\XXX^T(\VV\VV^T)^{-1}\VV\left(\xiTerm + \eTilde\right) \right)\\
    =& \qTwo + (\ZZZ\ZZZ^T)^{-1}\ZZZ\bm{\gamma}\ \text{ (recall the definition of $\bm{\gamma}$ in \cref{eq.def_gamma})}.
\end{align*}
Thus, we have
\begin{align}
    \normTwo{\qTwo-\qTilde}^2 = \normTwo{(\ZZZ^T\ZZZ)^{-1}\ZZZ\bm{\gamma}}^2.\label{eq.temp_042323}
\end{align}
We have
\begin{align}
    \normTwo{(\ZZZ^T\ZZZ)^{-1}\ZZZ\bm{\gamma}}^2 \leq \frac{\normTwo{\bm{\gamma}}^2}{\lambda_{\min}^2(\ZZZ)}\ \text{ (by \cref{le.norm_min_eig})}.\label{eq.temp_0412321}
\end{align}
By \cref{le.singular_Gaussian} and \cref{as.Gaussian}, we have
\begin{align}
    \Pr\left\{\lambda_{\min}(\ZZZ)\geq \sqrt{\nTwo}-\sqrt{\pSpecial{2}}-\sqrt{2\log \pSpecial{2}}\right\}\geq 1-\frac{2}{\pSpecial{2}}.\label{eq.temp_0412322}
\end{align}
By \cref{eq.temp_042323,eq.temp_042305,eq.temp_0412321,eq.temp_0412322} and the union bound, we have
\begin{align*}
    \Pr\left\{\normTwo{\qTwo-\qTilde}^2 \leq \frac{\CC}{\left(\sqrt{\nTwo}-\sqrt{\pSpecial{2}}-\sqrt{2\log \pSpecial{2}}\right)^2}\right\}\geq 1 - \frac{10}{\min \{\nOne,\nTwo,\pCommon,\pSpecial{2}\}}.
\end{align*}
The result of the underparameterized fine-tuning regime thus follows.


\subsection{Proof of Lemma~\ref{le.fine_CC}}\label{subsec.proof_fine_CC}
\begin{lemma}\label[lemma]{le.kTilde}
When $\pCommon > 4286$ and $\frac{\pCommon}{\nSum}\leq \frac{1}{7}$, we have $\kTilde\leq \frac{1}{6}$.
% \begin{align*}
%     \Pr\left\{\right\} \text{ if }\pSpecial{2} \geq 100 \nTwo,
% \end{align*}
% and
% \begin{align*}
%     \Pr\left\{\right\}\geq \ \text{ if }.
% \end{align*}
\end{lemma}
\begin{proof}
Because $\frac{\pCommon}{\nSum}\leq \frac{1}{7}$ and recalling the definition of $\kTilde$ in \cref{eq.def_kTilde}, we have
\begin{align}
    \kTilde= & \frac{\frac{\pCommon}{\nSum}+2\sqrt{\frac{\pCommon}{\nSum}\frac{\ln \pCommon}{\nSum}}+2\frac{\ln \pCommon}{\nSum}}{1-2\sqrt{\frac{\ln \nSum}{\nSum}}}\\
    \leq & \frac{\frac{\pCommon}{\nSum}+2\sqrt{\frac{\pCommon}{\nSum}\frac{\ln \nSum}{\nSum}}+2\frac{\ln \nSum}{\nSum}}{1-2\sqrt{\frac{\ln \nSum}{\nSum}}}\ \text{ (since $\pCommon\leq \nSum$)}\\
    \leq &\frac{\frac{1}{7}+ 2\sqrt{\frac{1}{7}a}+2a}{1 - 2\sqrt{a}}\ \text{ (since $\frac{\pCommon}{\nSum}\leq \frac{1}{7}$)},\label{eq.temp_043001}
\end{align}
where $a\defeq \frac{\ln \nSum}{\nSum}$.

Since $\pCommon > 4286$ and $\frac{\pCommon}{\nSum}\leq \frac{1}{7}$, we have $\nSum> 7 \times 4286 > 30000$. Thus, we have $a \leq \frac{\ln 30000}{30000}$ (since $\frac{\ln \nSum}{\nSum}$ is monotone decreasing w.r.t. $\nSum$ when $\nSum > e$). Noticing that the right-hand-side of \cref{eq.temp_043001} is monotone decreasing w.r.t. $a$, we thus have
\begin{align*}
    \kTilde \leq \frac{\frac{1}{7}+ 2\sqrt{\frac{1}{7}\frac{\ln 30000}{30000}}+2\frac{\ln 30000}{30000}}{1 - 2\sqrt{\frac{\ln 30000}{30000}}}\approx 0.1636 \leq \frac{1}{6}.
\end{align*}
% import numpy as np
% n = 30000
% a = np.log(n) / n
% r = (1 / 7 + 2 * np.sqrt(1 / 7 * a) + 2 * a) / (1 - 2 * np.sqrt(a))
% print(r)
\end{proof}

\begin{lemma}\label[lemma]{le.5000}
When $\nOne,\nTwo\geq 5000$, we have
\begin{align}
    & \nOne+2\sqrt{\nOne\ln \nOne}+2\ln \nOne\leq 1.1\nOne,\label{eq.temp_043011}\\
    & \nTwo+2\sqrt{\nTwo\ln \nTwo}+2\ln \nTwo \leq 1.1\nTwo,\label{eq.temp_043012}
\end{align}
\end{lemma}
\begin{proof}
Define a function $f(x)=2\sqrt{\frac{\ln x}{x}} + 2\frac{\ln x}{x}$. Since $\frac{\ln x}{x}$ is monotone decreasing when $x > e$, when $x \geq 5000$, we have
\begin{align*}
    f(x)\leq f(5000)\approx 0.086\leq 0.1.
\end{align*}
Thus, when $\nOne \geq 5000$, we have
\begin{align*}
    &2\sqrt{\frac{\ln \nOne}{\nOne}} + 2\frac{\ln \nOne}{\nOne} \leq 0.1\\
    \implies & 2\sqrt{\nOne \ln \nOne}+2\ln \nOne \leq 0.1 \nOne\\
    \implies & \text{\cref{eq.temp_043011}}.
\end{align*}
Similarly, we can get \cref{eq.temp_043012}. The result of this lemma thus follows.
% import numpy as np
% x = 5000
% a = np.log(x) / x
% r = 2 * np.sqrt(a) + 2 * a
% print(r) 
\end{proof}

Now we are ready to prove \cref{le.fine_CC}.
\begin{proof}[Proof of \cref{le.fine_CC}]
We have
\begin{align*}
    &\text{\cref{eq.requirement}}\\
    \implies & \frac{\nOne}{\nTwo}\left(\kTilde \sigmaOne^2 + \kTilde \normTwo{\qOne}^2+\similarity^2\right)+\sigmaTwo^2 + \kTilde \sigmaTwo^2 + \kTilde \normTwo{\qTwo}^2 \leq \left(0.01 + \frac{1}{6}\right) \normTwo{\qTwo}^2\\
    & \ \text{ (since $\kTilde\leq \frac{1}{6}$ by \cref{le.kTilde})}\\
    \implies & 3.3 \left(\frac{\nOne}{\nTwo}\left(\kTilde \sigmaOne^2 + \kTilde \normTwo{\qOne}^2+\similarity^2\right)+\sigmaTwo^2 + \kTilde \sigmaTwo^2 + \kTilde\normTwo{\qTwo}^2\right) \leq \frac{0.2+3.3}{6}\normTwo{\qTwo}^2\\
    & \ \text{ (since $\frac{0.2}{6}\approx 0.03333\geq 0.01 \times 3.3$)}\\
    \implies & 3.3 \nOne \left(\kTilde \sigmaOne^2 + \kTilde \normTwo{\qOne}^2+\similarity^2\right) + 3.3\nTwo \left(\sigmaTwo^2 + \kTilde \sigmaTwo^2 + \kTilde\normTwo{\qTwo}^2\right) \leq \frac{7\nTwo}{12}\normTwo{\qTwo}^2\\
    \implies & \CC \leq  \frac{7\nTwo}{12}\normTwo{\qTwo}^2\ \text{ (by \cref{le.5000} and \cref{eq.def_CC})}.
\end{align*}
The result of this lemma thus folllows.
\end{proof}
